Learning Fine Scale Dynamics from Coarse Observations via Inner Recurrence

Recent work has focused on data-driven learning of the evolution of unknown systems via deep neural networks (DNNs), with the goal of conducting long term prediction of the dynamics of the unknown system. In many real-world applications, data from time-dependent systems are often collected on a time scale that is coarser than desired, due to various restrictions during the data acquisition process. Consequently, the observed dynamics can be severely under-sampled and do not reflect the true dynamics of the underlying system. This paper presents a computational technique to learn the fine-scale dynamics from such coarsely observed data. The method employs inner recurrence of a DNN to recover the fine-scale evolution operator of the underlying system. In addition to mathematical justification, several challenging numerical examples, including unknown systems of both ordinary and partial differential equations, are presented to demonstrate the effectiveness of the proposed method.

==> Chaotic.tex <==
\subsection{Example 2: Chaotic System with Missing Variables}

Next we consider a chaotic system that is only partially observed. That is, while the full system is given by
\[ \begin{cases} 
      \dot{x}_1 = -x_2-x_3,\\
      \dot{x}_2 = x_1+\frac15 x_2,\\
      \dot{x}_3 = \frac15 + y - 5x_3,\\
      \dot{y} = -\frac{y}{\epsilon} + \frac{x_1x_2}{\epsilon},
   \end{cases}
\]
with $\epsilon=0.01$, only $\mathbf{z} = (x_1,x_2,x_3)^T$ are observed. Training data are collected by sampling uniformly over the computational domain of $[-7.5,10]\times[-10,7.5]\times[0,18]\times[-1,100]$. A ResNet structure with 3 hidden layers with 30 nodes each and memory length $n_M=60$ is used, as in \cite{FuChangXiu_JMLMC20}. The mean squared loss function is minimized using Adam with a constant learning rate of $10^{-3}$.

In all, 1000 individual models are trained for 100 epochs each. As a reference, prediction with each individual model is carried out for one time step using the new initial condition $\mathbf{z}_0=(-3.7634,7.1463,13.1806)^T$ (along with $n_M$ memory) in order to look at the distribution of the local truncation error. Table \ref{table:ex2_chaotic} show the biases and variances of the local truncation errors for the individual models in the $K=1$ (i.e. no ensemble) column.

Next, 500 ensemble models of size $K=50$ are chosen via sampling with replacement from the 1000 individual DNN models, and one-step ensemble averaged prediction is carried out using the same initial condition. As in Ex. 1, Table \ref{table:ex2_chaotic} shows that the biases are not affected by ensemble averaging, while the variances of the $K=50$ ensemble models are roughly $1/K$ of that of the individual models. In addition, Table \ref{table:ex2_chaotic} shows the mean squared local truncation error (MSE) in each state variable, computed as in \eqref{mse1} and \eqref{mse2}. We see that since bias is squared in the formula, that variance dominates the MSE and so this total numerical error also exhibits a roughly $1/K$ scaling.

Figure \ref{fig:chaotic_histogram} shows the distributions of the local truncation errors in each of the observed variables in histograms compared with a normal distribution with corresponding biases and variances from Table \ref{table:ex2_chaotic}. For all three observed variables, the local truncation errors fail to reject a chi-square goodness-of-fit test with null hypothesis that the errors come from a Gaussian distribution with the corresponding bias and variance at $0.05$ significance level. This demonstrates the scalar version of \eqref{local_WA} in this case.



==> PDE.tex <==
\subsection{Example 3: Partial Differential Equation System} \label{sec:pdesystem}

%for a system of PDEs with state variables
%$U=(u_1,\dots, u_L)$ and governed by unknown PDE system
%\be
%\partial_t u_i = \mathcal{L}_i(U), \qquad i=1,\dots, L,
%\ee
%where the PDE operator $\mathcal{L}_i$ includes partial derivatives of
%$U$. Our DNN model \eqref{NN_map} for scalar PDE \eqref{PDE}, as illustrated in Figure
%\ref{fig:basic_NN}, can be extended to the system by merely
%concatenating all the state variables into a single larger
%vector. That is,
%let $\u_i\in \R^N$ be the data snapshot of each component $u_i$, $i=1,\dots,
%L$. We then define
%\be
%\U = [\u_1^T, \cdots, \u_L^T]^T\in \R^{N L}
%\ee
%as the concatenated state vector. The DNN structure and network model
%in the previous sections can then be applied directly to $\U$.

%Note that it is possible, and maybe even preferable mathematically, to
%construct a more ``refined'' DNN structure to apply to each of the
%PDEs in the system. However, our early numerical experimentation
%indicated that the straightforward concatenation approach is a
%flexible numerical approach. Further refinement in DNN structure for
%PDE systems will be investigated in a future study.

Finally, we discuss the proposed ensemble averaged DNN learning for systems of PDEs. As in \cite{chen2022deep}, we consider the linear wave system
\begin{align}\label{eq:vecsystem}
\mathbf{u}_t = \A\mathbf{u}_x, { \quad x \in [0,2\pi],}
\end{align}
where
\begin{align*}
\mathbf{u} = \begin{bmatrix} u_1(x,t) \\ u_2(x,t)\end{bmatrix} \quad\text{and}\quad \A=\begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix},
\end{align*}
with $2\pi$-period boundary condition. (Note that even though its
form is simple, linear wave equations like this are exceptionally
difficult to solve accurately using numerical methods.)
Training data are collected over a uniform grid with $N=50$ points by computing
%and $n_L=10$ steps with a time step $\Delta t = 0.01$.
%They are
the exact solution of the
true system under randomized initial conditions in the form of the
Fourier series
\begin{equation} \label{Fourier}
	u(x,0) = a_0+ \sum_{n=1}^{N_c} \left ( a_n\cos(nx) +
          b_n\sin(nx) \right ).
\end{equation}
In particular, the initial conditions for
both components $u_1$ and $u_2$ are generated by sampling
\eqref{Fourier} with $a_0\sim U[-\frac{1}{2},\frac{1}{2}]$, and
$a_n ,b_n\sim U\left[-\frac{1}{n} ,\frac{1}{n}\right]$ for $1\le n \le N_c=10$. 
%A total of $10,000$ trajectories are generated for the training data set.
The DNN structure consists of an input layer with $100$ neurons, to
account for the two components $u_1$ and $u_2$, each of which has $50$
spatial nodes. The disassembly block has dimension $100\times 1 \times 5$ and the
assembly layer has dimension $1\times1\times 5$, as in \cite{chen2022deep}. 
The mean squared loss function is minimized using Adam with a constant learning rate of $10^{-3}$.
%Hyperbolic tangent is used as the activation function for each layer.

In all, 1000 individual models are trained for 40 epochs each. 
As a reference, prediction with each individual model is carried out for one time step using the new initial condition
\begin{align*}
\mathbf{u}(x,0) &= \begin{bmatrix} \exp(\sin(x)) \\ \exp(\cos(x)) \end{bmatrix}.
\end{align*}
Since in this case the large spatial grid results in 100 state variables, the 2-norm of the local truncation errors in $\u$ are computed.
Table \ref{table:ex3_pde} shows the bias and variance of these normed local truncation errors for the individual models in the $K=1$ (i.e. no ensemble) columns.

Next, 500 ensemble models each of sizes $K=2,5,10$ are chosen via sampling with replacement from the 1000 individual DNN models, and one-step ensemble averaged prediction is carried out for one time step using the same initial condition. Bias and variance are retrieved to summarize the distribution of the 2-norm of the local truncation errors. Table \ref{table:ex3_pde} shows consistency with the previous examples in that the biases are similar while the variances differ roughly by a factor of $1/K$. The mean squared normed local truncation error (MSE) is also computed. In this case, unlike Ex. 2, the squared bias actually dominates the MSE, yet this total numerical error still exhibits a roughly $1/K$ scaling.

%For $K=2$, 71 of 100 state variables fail to reject the null hypothesis of a normal distribution in a chi-square goodness of fit test. For $K=5$ and $K=10$, 88 and 93 of 100 fail to reject, respectively. This gives some sense of the convergence for \eqref{local_WA} in this example.

\begin{table}[h]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c| }
 \hline
% \diagbox{stat}{$K$} & 1 & 2 & 5 & 10 \\ 
$K$ & 1 & 2 & 5 & 10 \\ 
 \hline
$\textrm{Bias}(\|\u\|_2)$ & $6.2115\cdot10^{-3}$ & $4.5229\cdot10^{-3}$ & $2.8915\cdot10^{-3}$ & $2.1219\cdot10^{-3}$ \\ 
\hline
$\text{Var}(\|\u\|_2)$ & $5.6610\cdot 10^{-6}$ & $1.6189\cdot10^{-6}$ & $3.9791\cdot10^{-7}$ & $1.4576\cdot10^{-7}$ \\
\hline
$\text{MSE}(\|\u\|_2)$ & $4.4244\cdot 10^{-5}$ & $2.2075\cdot10^{-5}$ & $8.7588\cdot10^{-6}$ & $4.6482\cdot10^{-6}$ \\
 \hline
\end{tabular}
\end{center}
\caption{Ex. 3: Normed local truncation error statistics for size $K$ ensemble models.}
\label{table:ex3_pde}
\end{table}

